TorchRL: A data-driven decision-making library for PyTorch

PyTorch has ascended as a premier machine learning framework, yet it lacks a native and comprehensive library for decision and control tasks suitable for large development teams dealing with complex real-world data and environments. To address this issue, we propose TorchRL, a generalistic control library for PyTorch that provides well-integrated, yet standalone components. We introduce a new and flexible PyTorch primitive, the TensorDict, which facilitates streamlined algorithm development across the many branches of Reinforcement Learning (RL) and control. We provide a detailed description of the building blocks and an extensive overview of the library across domains and tasks. Finally, we experimentally demonstrate its reliability and flexibility and show comparative benchmarks to demonstrate its computational efficiency. TorchRL fosters long-term support and is publicly available on GitHub for greater reproducibility and collaboration within the research community. The code is open-sourced on GitHub.

==> old_neurips/paper_content.tex <==


\begin{abstract}

Striking a balance between integration and modularity is crucial for a machine learning library to be versatile and user-friendly, especially in handling decision and control tasks that involve large development teams and complex, real-world data, and environments.
To address this issue, we propose TorchRL, a generalistic control library for PyTorch that provides well-integrated, yet standalone components.
With a versatile and robust primitive design, TorchRL facilitates streamlined algorithm development across the many branches of Reinforcement Learning (RL) and control.
We introduce a new PyTorch primitive, TensorDict, as a flexible data carrier that empowers the integration of the library's components while preserving their modularity. Hence replay buffers, datasets, distributed data collectors, environments, transforms and objectives can be effortlessly used in isolation or combined.
%TorchRL makes the design and training of control algorithms accessible to any machine learning practitioner, thanks to a simple, efficient, and composable interface. 
We provide a detailed description of the building blocks, supporting code examples and an extensive overview of the library across domains and tasks. Finally, we show comparative benchmarks to demonstrate its computational efficiency. 
TorchRL fosters long-term support and is publicly available on GitHub for greater reproducibility and collaboration within the research community.
The code is opensourced on \hyperlink{https://github.com/pytorch/rl}{GitHub}.

\end{abstract}

\section{Introduction}

The advancements in hardware supporting machine learning (ML) training and deployment pipelines, along with the simultaneous release of robust ML libraries, provide a potent combination that can drive artificial intelligence (AI) forward. Originally, breakthroughs in AI were powered by custom code tailored for specific machines and backends. However, with the widespread adoption of AI accelerators like GPUs and TPUs, as well as user-friendly development frameworks such as PyTorch \cite{Paszke_PyTorch_An_Imperative_2019}, TensorFlow \cite{tensorflow2015-whitepaper}, and Jax \cite{jax2018github}, we have moved beyond this point. 

Deploying these technologies in the field of decision-making has been more challenging than in other AI domains, such as computer vision or natural language processing, where a few libraries have gained widespread recognition within their respective research communities. 
We attribute the slow progress to the dynamic requirements of decision-making algorithms, which creates a trade-off between modularity and component integration. 
% Diversity of algorithms forces libs to make a trade-off
The current solutions in this field are inadequate for accommodating the variety of applications, ranging from gaming to fine-tuning generative models with human feedback~\cite{NIPS2017_d5e2c0ad}, due to being either too high-level and difficult to repurpose across use cases or too low-level for non-experts to use practically. 
Because of this intricate landscape, a consensus adoption of frameworks within the research community remains limited~\cite{brockman2016openai}.
Nevertheless, we believe that moving forward, the next generation of libraries for decision-making will need to be easy to use and rely on widespread frameworks while still being powerful, efficient, scalable, and broadly applicable, to meet the demands of this rapidly evolving and heterogeneous field. This is the problem that TorchRL addresses.

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/torchrl.png}
  \caption{TorchRL overview. The left side showcases the key components of the library, demonstrating the data flow with TensorDict instances passing between modules. On the right side, a code snippet is provided as a toy example, illustrating the training of DDPG. The script provides users with full control over the algorithm's hyperparameters, offering a concise yet comprehensive solution. Still, replacing a minimal number of components in the script enables a seamless transition to another similar algorithm, like SAC or REDQ.}
  % \albert{Maybe clarify that the actor is generally the same python object? at least in the non-distributed case}
  \label{fig:1}
  \vspace{-5mm}
\end{figure}

% \matteo{I think here we can cut some stuff}
The ecosystem of decision-making algorithms is complex an encompasses very diverse applications such as gaming (\cite{mnih2013playing, Silver2016, Silver2017, Silver2018, alphastarblog,openai2019dota,espeholt2018impala}), robotic control \cite{tobin2017domain, Peng_2018,rudin2022learning,openai2019solving}, autonomous driving \cite{Aradi2020,Sallab_2017}, finance \cite{ganesh2019reinforcement,Hambly2021,Mosavi2020}, bidding in online advertisement \cite{Jin_2018,Cai2017,zou2019reinforcement,zhu2021deep}, cooling system control \cite{luo2022controlling}, faster matrix multiplication algorithms \cite{Fawzi2022}, chip design \cite{Mirhoseini2021} and drug synthesis \cite{Popova_2018}, among many others.
RL is also a powerful tool to help train other models through AutoML solutions \cite{He_2018_ECCV,zoph2017neural,zoph2018learning,baker2017designing,zhong2018practical} or incorporate human feedback in generative model fine-tuning \cite{christiano2017deep,leandro_von_werra_2023_7790115,WebGPT}. 
The available toolbox is extensive, including techniques such as sim-to-real transfer \cite{tobin2017domain, Peng_2018,rudin2022learning,openai2019solving}, model-based RL \cite{brunnbauer2022latent,wu2022daydreamer,hansen2022modem,hansen2022temporal} or offline data collection for batched RL and imitation learning \cite{kalashnikov2018qtopt,shah2022offline}.
In addition, algorithms and training pipelines must often meet challenging scaling requirements, such as distributed inference \cite{mnih2016asynchronous,espeholt2018impala} or distributed model execution \cite{WebGPT}. They must also satisfy imperative deployment demands when used on hardwares like robots or autonomous cars, which often have limited computational resources and need to operate in real time.

Training decision-making models involves a sequential and algorithmic process, where the cooperation between framework components is vital for adaptability across different applications.
Actors, collectors or replay buffers need to be able to handle various modalities.
Imposing a fixed input/output format would restrict their reusability, while eliminating all restrictions would create significant difficulties in designing adaptable scripts. 
Consequently, conventional decision-making libraries must choose between a well-integrated framework with a high-level API or a flexible framework with basic building blocks of limited scope.
The former hinders quick coding and testing of new ideas, while the latter leads to complex code and a poor user experience. 
TorchRL elegantly tackles each of these challenges in a comprehensive and flexible manner.

In this paper, we will explain our approach to overcoming these challenges by focusing primarily on the problem of module portability, communication and code repurposing.
We introduce TensorDict, a new PyTorch data carrier, which is central to achieving this goal.
By adopting this new coding paradigm, we demonstrate how simple it is to reuse ML scripts and primitives across different tasks or research domains.
Building upon this innovative technical foundation, we explore various independent components that rely on this abstraction.
These components encompass a range of advanced solutions, including distributed data collectors, cutting-edge models like Decision Transformers, and highly specialized classes such as an environment API compatible with single and multi-agent problems.
We demonstrate that the current state of the library encompasses diverse categories of decision-making algorithms, caters to a wide range of applications, performs optimally on both small-scale machines and large clusters, and demands minimal technical knowledge and effort to get started.

%\subsection{Related work}
\textbf{Related work.}
Currently, there is a vast array of libraries available for reinforcement learning. Many of these libraries offer a limited selection of implemented algorithms, such as Dopamine \cite{castro18dopamine}, ChainerRL \cite{JMLR:v22:20-376}, PyTorchRL \cite{bou2022efficient}, TFAgents \cite{TFAgents}, RLkit and autonomous-learning-library \cite{nota2020autonomous}. Other libraries are specifically designed for particular niches, such as Pyqlearning, Openspiel \cite{LanctotEtAl2019OpenSpiel} and Facebook/ELF \cite{tian2017elf}. There are also libraries that only support a small number of environments, like OpenSpiel and reaver \cite{reaver}, or that lack the capability for parallel environments with distributed learning, such as MushroomRL \cite{JMLR:v22:18-056}.
Additionally, some previously popular libraries have fallen out of favor and are no longer actively maintained, including Tensorforce \cite{tensorforce}, KerasRL \cite{plappert2016kerasrl}, rlpyt \cite{DBLP:journals/corr/abs-1909-01500}, ReAgent \cite{gauci2018horizon} and IntelLabs/coach \cite{caspi_itai_2017_1134899}. % Given the wide range of options available, it is sensible to narrow our focus to a few select libraries that can be effectively compared to TorchRL. For this purpose, the following libraries have been chosen.

Currently, popular solutions often prioritize high-level approaches that favor component integration. This is particularly necessary for libraries that provide non-standalone components or that rely on limited data carriers, as they require additional code to ensure seamless integration between components. This is the case of Stable-baselines (and Stable-baselines3, SB3) \cite{JMLR:v22:20-1364}, ElegantRL \cite{erl}, Acme \cite{hoffman2020acme}, DI-engine \cite{ding}, garage \cite{garage} or RLlib~\cite{liang2018rllib}. Some of these libraries are compatible with more than one deep learning framework and even allow for distributed training. Others focus on letting researchers compare against pre-existing baselines.
Another popular resource with some similarities to TorchRL is Tianshou \cite{tianshou}, which offers a large coverage of RL algorithms, high engineering quality standards, a generic data carrier and modular components. However, it does not offer standalone components that can be used independently from the rest of the library. Tianshou's focus is to provide pytorch-first RL trainers that cover a wide range of algorithms, making it easy to solve a given problem with RL without requiring an extensive domain knowledge.
Finally, CleanRL\cite{huang2022cleanrl} offers Torch and JAX efficient single-file implementations of RL algorithms. This design choice simplifies code comprehension, enhancing its clarity. However, a notable drawback of this approach is the lack of component reusability, which poses a significant challenge to scaling any project without extensive code duplication.

In Appendix H, we detail how TorchRL design choices complements other existing libraries and make it a fit to be used as a backend for other PyTorch-based RL libraries, with a focus on its modularity and communication protocols which are the defining features of our framework.

\section{TorchRL's data carrier}
\label{sec:data_carrier}

TorchRL is built on the fundamental concept of self-contained independent components.
The resulting atomicity and modularity facilitate versatile usage of individual components within most machine learning workflows.
In \autoref{fig:1} we outline TorchRL's general organization. 
In this section, we highlight the importance of a  data carrier that enables seamless communication between these components. 
To address this need, we introduce our solution, the \textit{TensorDict} class, which serves as an intuitive and versatile means of data exchange.
Additionally, we provide an overview of the key components in the library, which can be used independently or as foundational elements for constructing decision-making algorithms, as depicted in \autoref{fig:1}.

\textbf{Inter-class communication in decision-making workflows.}


\input{sections/components/tensordict}


\section{TorchRL  components}
\label{sec:modules}
%In the following, we introduce the components of TorchRL, which are kept modular and interconnected using TensorDict. 


\paragraph{Environment API, wrappers, and transforms.}
\label{sec:env}
\input{sections/components/env_wrappers}

\textbf{Data collectors.}
\input{sections/components/data_collectors}
%\albert{Maybe modules should be introduced before collectors? since collectors need to use an actor}

\textbf{Replay buffers and datasets.}
\input{sections/components/data_utilities}

\textbf{Modules and models.}
\input{sections/components/modules}

\textbf{Objectives and value estimators.}
\input{sections/components/objectives_and_value_estimators}

\textbf{Trainers.}
\input{sections/components/trainers}

\section{Ecosystem}
To flourish a thriving community around the library, in addition to open-sourcing the library, we are committing to designing a comprehensive ecosystem to support our users. The ecosystem comprises documentation, datasets, issues-tracking, model library, sample use cases, etc. Below we detail a few of these modules and refer the readers to our webpage for further information.

\begin{threeparttable}[ht!]
  \caption{GAE efficiency. The data consisted of a batch of 1000 trajectories of 1000 time steps, with a "done" frequency of 0.001, randomly spread across the data.} 
  % #Whenever possible, operations were executed on an A100 GPU.}
  \label{gae-efficiency}
  \centering
  \begin{tabular}{llllllll}
    \toprule
    Library     & Speed (ms)    & Standalone & Meta-RL & Adjacent\tnote{\$} & Backend & Device\\
    \midrule
    Tianshou\tnote{$\dagger$} & 5.15 & - & - & + & namba & CPU \\
    SB3\tnote{$\dagger$} & 14.1 & - & - & + & numpy & CPU \\
    RLLib (Ray)\tnote{*} \> \tnote{$\dagger$} & 9.38 & - & - & - & scipy & CPU \\
    CleanRL & 1.43 & - & - & + & Jax & GPU \\
    TorchRL-compiled & 2.67 & + & + & +  & PyTorch & GPU  \\
    TorchRL-vec & \textbf{1.33} & + & + & + & PyTorch & GPU  \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
    \item[\$] Using Tianshou's implementation requires transforming tensors to numpy arrays and then transforming the result back to tensors. This overehead is not accounted for here.
    \item[*] A proper usage of Ray's GAE implementation would have needed a split of the adjacent trajectories, which we did not do to focus on the implementation efficiency.
    \item[$\dagger$] Numpy or similar backends require moving data from and to GPU which can substantially impact performance. Those data moves are unaccounted for in this table but can double the GAE runtime.  \end{tablenotes}
\end{threeparttable}

\vspace{0.25cm}
\textbf{Documentation, knowledge-base, engineering. }\input{sections/components/doc}

\textbf{Applications. } \input{sections/marl}


% \subsection{Comparison of design decisions}
% \vk{I propose that move this to appendix. This is a mix of what is commonly found in related works and experiment section. }
% \input{sections/components/design}
%\matteo{Is there a reason related works are between methods and experiments?}
%\vince{happy to move it somewhere else but yes there is: we want to say "tensordict is cool" etc but it's hard if ppl don't know what we're talking about. So it's easier to compare ourselves once we have set the stage clearly. It is not a no-no IMO...}
%\matteo{got it, and we also need it before experiments since we are comparing}



 


\section{Experiments}

\textbf{Compute efficiency.}
To check that our solution does not come at the cost of reduced throughput, we test two selected functionalities (advantage computation and data collection) against other popular libraries. These experiments were run on an AWS cluster with a single node (96 CPU cores and 8 A100 GPUs). These results are reported in \autoref{gae-efficiency} and \autoref{collector-efficiency}. Overall, these results show that our solutions have a comparable if not better throughput than others and in general a greater coverage of functionalities.

\begin{threeparttable}[ht!]
  \caption{Data collection speed on the \pyth{"PongNoFrameskip-v4"} environment. In each case, a random policy was used.}
  \label{collector-efficiency}
  \centering
  \begin{tabular}{llll}
    \toprule
    Library     & Speed (fps)  & Standalone collector & Environment Compatibility \\
    \midrule
    Tianshou\tnote{$\dagger$} & 7272 & + & Gym \\
    SB3\tnote{$\ddag$} & 1070 & - & Gym \\
    RLLib\tnote{$\dagger$} & 1167  & - & Any \\
    CleanRL\tnote{$\ddag$} & 3670  & + & Gym \\
    TorchRL (sync) \tnote{\$}\;\tnote{$\dagger$} & 2991  & + & Any \\
    TorchRL (sync-preempted) \tnote{\$}\;\tnote{$\dagger$} & 3733  & + & Any \\
    TorchRL (async) \tnote{\$}\;\tnote{$\dagger$} & \textbf{8845}  & + & Any \\
    \bottomrule
  \end{tabular}
   \begin{tablenotes}
    \item[\$] Async collection means that the collector delivers the data on a first-ready-first-served basis. In the sync scenario, the collector waits for each worker to be ready before delivering the data. Our collectors also have a preemption mechanism to temper the effect of slower workers. In the corresponding example, a preemption threshold of 0.7 was used.
    \item[$\dagger$] We used 32 parallel processes, returning a total of 320 steps per batch. Depending on the (a)sync nature of the collection, this quantity was gathered from a single process or combined from all.
    \item[$\ddag$] Use vectorized environments from Gym or a version inherited from them.
\end{tablenotes}
\end{threeparttable}

\vspace{0.2cm}
\textbf{Algorithm evaluation.}
TorchRL equips its users with an extensive selection of example scripts that demonstrate cutting-edge algorithms for both online and offline RL. In order to ascertain the completeness and effectiveness of TorchRLs framework components, we provide documented validations of a variety of algorithms in Appendix F and G.

\section{Conclusion}

We have presented TorchRL, a modular decision-making library with composable, single-responsibility building pieces that rely on TensorDict for an efficient class-to-class communication protocol.
TorchRL's design principles are tailored for the dynamic field of decision making, enabling the implementation of a wide range of algorithms.
Furthermore, these design principles support the seamless integration of future innovations as new TensorDict compatible objects.
We believe TorchRL can be of particular interest to researchers and developers alike.
Its key advantage is that researchers can create or extend existing classes on their own and seamlessly integrate them with existing scripts without the need to modify the internal code of the library, allowing for quick prototyping while maintaining a stable and reliable code base.
We believe this feature will also be suited for developers looking to apply an AI solution to a specific problem, even if unaccounted for by the library: unlike the Agent classes commonly found in other libraries, TorchRL's design gives users fine-grained control over every aspect of training which we believe to be necessary to push decision-making research and applications to the next frontiers.
We demonstrate that TorchRL not only benefits from a wide range of functionalities but also exhibits computational efficiency.
The library is currently fully functional, and we are extensively testing it across various scenarios and applications.
We look forward to receiving feedback and aim to provide support and further enhance the library based on the input we receive.

% \vk{Add (1) a statement to support our claims in term of speed and efficiency via a head to head comparisions with other libraries.  Another to say that we validate the modularity by impletementing a variety of algos with competitive performance. (2) Add library is fully functional. We are doing extensive user testing. Curently we have XX external projects using the library. We hope to support and grow as more feedback trickles in.}

==> sections/components/trainers.tex <==
The modularity of TorchRL's components allows developers to write training scripts with explicit loops for data collection and neural network optimization in the traditional structure adopted by most ML libraries.
While this enables practitioners to keep tight control over the training process, it might hinder TorchRL's adoption by first-time users looking for one-fits-all solutions.
For this reason, we introduce a \pyth{Trainer} class that abstract this further complexity.
By exposing a simple \pyth{train()} method, trainers take care of running data collection and optimization while providing several hooks (i.e., callbacks) at different stages of the process.
These hooks allow users to customize various aspects of data processing, logging, and other training operations.
Trainers also encourage reproducibility by providing a checkpointing interface that allows to abruptly interrupt and restart training at any given time while saving models and RB of any given size.
An example of the \pyth{Trainer} class usage is provided in Appendix E.

% As shown in \autoref{fig:trainers}, they provide an additional option for consolidated training aimed at simplifying RL to the general public.
% \begin{figure}[tb]
%     \begin{subfigure}{0.46\linewidth}
% \begin{python}
% env = Env(...)
% qnet = QNet(...)
% collector = Collector(env, qnet)
% loss = Loss(qnet)
% for data in collector:
%     loss_data = loss(data)
% \end{python}
%     \caption{Modular training.}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.46\linewidth}
% \begin{python}
% trainer = Trainer(env_name, model_name)
% trainer.train()
% \end{python}
%     \caption{Consolidated training.}
%     \end{subfigure}
% \caption{The two training flavours in TorchRL. \matteo{the idea of this fig was to have a side by side comparison of how we train  vs w black box trainers. @vince maybe you can adjust the pseudo code a bit. We can also remove this for space}}
% \label{fig:trainers}
% \end{figure}
